Fix your downsampling ASAP! Be natively more robust via Aliasing and Spectral Artifact free Pooling

Convolutional Neural Networks (CNNs) are successful in various computer vision tasks. From an image and signal processing point of view, this success is counter-intuitive, as the inherent spatial pyramid design of most CNNs is apparently violating basic signal processing laws, i.e. the Sampling Theorem in their downsampling operations. This issue has been broadly neglected until recent work in the context of adversarial attacks and distribution shifts showed that there is a strong correlation between the vulnerability of CNNs and aliasing artifacts induced by bandlimit-violating downsampling. As a remedy, we propose an alias-free downsampling operation in the frequency domain, denoted Frequency Low Cut Pooling (FLC Pooling) which we further extend to Aliasing and Sinc Artifact-free Pooling (ASAP). ASAP is alias-free and removes further artifacts from sinc-interpolation. Our experimental evaluation on ImageNet-1k, ImageNet-C and CIFAR datasets on various CNN architectures demonstrates that networks using FLC Pooling and ASAP as downsampling methods learn more stable features as measured by their robustness against common corruptions and adversarial attacks, while maintaining a clean accuracy similar to the respective baseline models.

==> fig_adv_vs_base_trained.tex <==
\begin{figure}[t]
\caption[]{%
Spectrum of perturbed images, attacked by AutoAttack \cite{auto_attack} on differently trained ResNet-18 models: conventional (second row), our FLC Pooling (third row), and our ASAP (fourth row).
The center column depicts the spectrum of the perturbed image (left column), while the right column depicts the difference between the spectrum of the unperturbed image (first row) and the corresponding perturbed image.
The spectrum of the perturbed images between adversarially trained and conventionally trained networks differ, while the difference between different models is minor.
}
\begin{center}
\setlength\tabcolsep{1.5pt} 
\begin{tabular}{cccc@{\hskip 0.2in}ccc}
  \multicolumn{4}{c}{\small \textbf{Conventionally Trained} }    &   \multicolumn{3}{c}{\small \textbf{Adversarially Trained}} \\
  & {\scriptsize Example} & {\scriptsize Spectrum} &  & {\scriptsize Example} & {\scriptsize Spectrum} &  \\
  % & & & {\scriptsize Difference} &  & & {\scriptsize Difference} \\
{\scriptsize\rotatebox{90}{Original}}
& \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_1.pdf}
& \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_2.pdf}
& %\includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_3.pdf}
{\scriptsize \makecell{Spectrum \\ Difference}}
& \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_1.pdf} 
& \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_2.pdf}
& %\includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_3.pdf}
{\scriptsize \makecell{Spectrum \\ Difference}}
\\
{\scriptsize\rotatebox{90}{Baseline}} &
 \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_4.pdf} &
\includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_5.pdf} & \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_6.pdf} & \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_4.pdf} &
\includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_5.pdf} & \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_6.pdf} 
\\
{\scriptsize\rotatebox{90}{FLC (ours)}} &
 \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_7.pdf} &
\includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_8.pdf} & \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_9.pdf} & \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_7.pdf} &
\includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_8.pdf} & \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_9.pdf} 
\\
{\scriptsize\rotatebox{90}{ASAP(ours)}} &
 \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_10.pdf} &
\includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_11.pdf} & \includegraphics[width=0.13\linewidth]{conv_auto_attack_example_image10_Airplane_12.pdf} & \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_10.pdf} &
\includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_11.pdf} & \includegraphics[width=0.13\linewidth]{fgsm_auto_attack_example_image10_Airplane_12.pdf} 
\end{tabular}
\label{fig:adv_vs_base_trained}
\end{center}
\end{figure}

==> fig_aliasing_zebra.tex <==
\begin{figure}[t]%
\centering
\includegraphics[width=\columnwidth]{zebra_aliasing.pdf}
\caption{Example of aliasing after standard downsampling via striding compared to our anti-aliasing methods, FLC Pooling. Strided downsampling incorporates severe gird artifacts aka. aliasing artifacts.
}\label{fig:aliasing}
\end{figure}




==> fig_heart_abliation.tex <==
\begin{figure}[t]%
\centering
\includegraphics[width=\columnwidth]{heart_stepbystep_wops_abliation_onepaddingASAP_naming.pdf}
\caption{We compare different methods to strengthen our ASAP. First, we reduce spectral artifacts by a Hamming window and stabilized FFT \textcolor{orange}{($\text{ASAP}_{\textrm{stbl}}$)}. The second and third row show our ASAP including a Hamming filter and large asymmetric padding \textcolor{orange}{($\text{ASAP}_{\textrm{lp}}$)} (second row) or small asymmetric padding \textcolor{orange}{($\text{ASAP}_{\textrm{sp}}$)} (third row).
}\label{fig:heart_abliation}
\end{figure}




==> fig_ps_diff_mean_std.tex <==
\begin{figure}[t]%
\centering
\includegraphics[width=\columnwidth]{mean_std_ps_difference_asap.pdf}
\caption{Mean (blue) and standard deviation (red) of the power spectrum difference measured via KL divergence after downsampling with different downsampling methods over 1000 images of CIFAR10. %\textcolor{orange}{use other measure like MSE instead of KL DIV as we do not have a probability distribution and due to numerical instabilities can also not normalize to one}
}\label{fig:ps_diff}
\end{figure}




==> fig_time_fft_stbl_sp_lp.tex <==
\begin{figure}[t]
	\begin{center}
	\includegraphics[width=0.95\linewidth]{stbl_sp_lp_ffttime2832_std.pdf}
	\caption[]{Mean execution time and standard deviation over 10 independent runs each with 100 runs of our ASAP variants for images of size 28x28 versus size 32x32 on a Nvidia TITAN V. For images of size 32x32 (i.e.~$2^5\times 2^5$), ASAP$_\textrm{stbl}$ is faster than ASAP$_\textrm{sp}$. For array size 28x28, both are equally fast as expected.}
	\label{fig:time2832}
	\end{center}
\end{figure}

\begin{figure}[t]
	\begin{center}
	\includegraphics[width=0.95\linewidth]{stbl_sp_lp_ffttime224256_std.pdf}
	\caption[]{Mean execution time and standard deviation over 10 independent runs each with 100 runs of our ASAP variants for images of size 224x224 versus size 256x256 on a Nvidia TITAN V. For images of size 256x256 (i.e.~$2^8\times 2^8$), ASAP$_\textrm{stbl}$ is faster than ASAP$_\textrm{sp}$. For array size 224x224, both are equally fast as expected.}
	\label{fig:time256}
	\end{center}
\end{figure}

==> tab_alexnet_ablation.tex <==
\begin{table*}[t]
\caption[]{Accuracy (in percentage) on clean samples, perturbed samples with FGSM~\cite{harnesssing} and PGD~\cite{pgd} as well as corrupted samples~\cite{hendrycks2019robustness} for AlexNet trained without adversarial training on CIFAR-10. Attacks are done with an epsilon of $\epsilon=1/255$ and corruption performance is reported as mean over all severities. 
For CIFAR-10 our ASAP and FLC Pooling outperform the baseline and show overall a high robustness against adversarial attacks and common corruptions. 
}
\begin{center}
\begin{tabular}{l|@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c}
\toprule
Architecture &  Acc@1 &  FGSM  &   PGD & Common Corruptions\\
\toprule
AlexNet \cite{Krizhevsky2012alexnet} &  \textbf{89.62} & 69.31 & 70.09 & 73.70
\\
FLC Pooling (ours) & 87.79 & 69.71 & 70.79 & \textbf{74.64} 
\\
$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) & 87.40 & 70.66 & 71.59 & 73.78
\\
$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & 87.83 & \textbf{71.24} & \textbf{72.14} & 73.54
\\
$\mathrm{ASAP}_{\mathrm{sp}}$(ours) &   87.43 & 70.22 & 71.38 & 73.97
\\
\bottomrule              
\end{tabular}
\label{tab:alexnet_ablation}
\end{center}
\end{table*}

==> tab_compare_adv_abl.tex <==
\begin{table*}[t]
\caption[]{Accuracy (in percentage) and standard deviation on clean samples, perturbed samples with FGSM~\cite{harnesssing} and PGD~\cite{pgd} as well as corrupted samples~\cite{hendrycks2019robustness} for ResNet-18 trained without adversarial training on CIFAR-10. Attacks are done with an epsilon of $\epsilon=1/255$ and corruption performance is reported as mean over all severities. 
}
\begin{center}
\begin{tabular}{l|@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c}
\toprule
Method     &   Acc@1 &  FGSM  &   PGD \\
\toprule
Baseline &  93.03 $\pm$ 0.13 & 78.62 $\pm$ 0.28 & 72.49 $\pm$ 0.67 \\ %  & 76.93  $\pm$ 0.45    \\
\midrule
DCT Conv \cite{lukasik2023improving} WD & 88.80 $\pm$     0.16 & 60.53 $\pm$   1.06 & 58.65 $\pm$   1.21 \\
DCT Conv \cite{lukasik2023improving} SD & 89.93 $\pm$   0.10 & 61.37 $\pm$ 0.51 & 59.40   $\pm$  0.74 \\
%DCT Conv \cite{lukasik2023improving} hyperparams  & 89.37 & 55.91 & 51.03 \\
\midrule
FLC Pooling (ours) %nonorm 
& 93.12 $\pm$ 0.19 & 78.92 $\pm$ 0.26 & 74.17 $\pm$ 0.60 \\ % &78.59 $\pm$ 0.29  \\
ASAP + stabilized FFT (ours) & 93.12 $\pm$ 0.25 & 79.08 $\pm$ 0.43 & \textbf{75.06 $\pm$ 0.76} \\ % & \textbf{78.68 $\pm$ 0.19}\\
ASAP + large padding (ours) & \textbf{93.24 $\pm$ 0.15} & \textbf{79.17 $\pm$ 0.23} & 74.94 $\pm$ 0.56 \\ % & 78.65 $\pm$ 0.33\\
ASAP + small padding (ours) &  93.00 $\pm$ 0.12 & 79.12 $\pm$ 0.49 & 74.69 $\pm$ 1.36 \\ %& 78.42 $\pm$ 0.20 \\

\bottomrule              
\end{tabular}
\label{tab:adv_abl}
\end{center}
\end{table*}

==> tab_compare_adv_abl_rn50.tex <==
\begin{table}[t]
\caption[]{Accuracy (in percentage) and standard deviation on clean samples, perturbed samples with FGSM~\cite{harnesssing} and PGD~\cite{pgd} for ResNet-50 trained without adversarial training on CIFAR-10 compared to the results reported in \cite{rodriguezmunoz2022driver}.
}
\begin{center}
\begin{tabular}{c|l|cc}
\toprule
 Attack     &  Method  &  FGSM  &   PGD \\
 Epsilon &  &  &\\
\toprule
&Anti-Aliasing \cite{rodriguezmunoz2022driver} & 87.44 &  87.44 \\
 &FLC Pooling (ours) & 94.06 & 94.06\\ %seed 42
0&$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) & 93.78 &  93.78\\ % seed 0
&$\mathrm{ASAP}_{\mathrm{sp}}$ (ours) & 93.68 & 93.68\\ % seed 44
&$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & \textbf{94.20  }& \textbf{94.20 }\\ % seed 43
\midrule
&Anti-Aliasing \cite{rodriguezmunoz2022driver} & 70.53 & 61.67 \\
 &FLC Pooling (ours) & 75.10 & 68.66\\
2&$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) & 73.46 &  68.89\\
&$\mathrm{ASAP}_{\mathrm{sp}}$ (ours) &  67.74 & 60.66\\
&$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & \textbf{74.99 }&  \textbf{71.61}\\
\midrule
&Anti-Aliasing \cite{rodriguezmunoz2022driver} & 56.85 & 25.71 \\
 &FLC Pooling (ours) & 71.28 & 52.60\\
4&$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) & 68.95 & 53.92 \\
&$\mathrm{ASAP}_{\mathrm{sp}}$ (ours) & 61.19 &  42.65 \\
&$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & \textbf{73.05 }& \textbf{69.13} \\
\midrule
&Anti-Aliasing \cite{rodriguezmunoz2022driver} & 39.91 & 5.65 \\
&FLC Pooling (ours) & 68.08 & 32.63\\
8&$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) & 63.20 &  31.20 \\
&$\mathrm{ASAP}_{\mathrm{sp}}$ (ours) & 54.14 &  16.99\\
&$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) &\textbf{71.50} & \textbf{57.34} \\ %seed43
\bottomrule              
\end{tabular}
\label{tab:adv_abl_rn50}
\end{center}
\end{table}

==> tab_compare_adv_abl_rn9.tex <==
\begin{table}[t]
\caption[]{Accuracy (in percentage) and standard deviation on clean samples, perturbed samples with FGSM~\cite{harnesssing} and PGD-40~\cite{pgd} and AutoAttack \cite{auto_attack} with an attack strength of $\epsilon=1/255$ for ResNet-9 trained without adversarial training on CIFAR-10 compared to the results reported in \cite{lukasik2023improving}.
}
\begin{center}
\begin{tabular}{@{}l|cccc@{}}
\toprule
 Method  & Clean  & FGSM  &   PGD & AA\\
\toprule
WD + Reg. \cite{lukasik2023improving} & 93.18 & 59.25 & 56.08 & 43.62\\
SD + Reg. \cite{lukasik2023improving} & 93.09 & 59.87 & 56.89 & 44.80 \\
\midrule
FLC Pooling (ours) & 94.58 & 69.21 & \textbf{67.03} & \textbf{56.96}\\ %seed 45
$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) & 94.64 & \textbf{69.27} & 66.03 & 55.23\\ %seed 45
$\mathrm{ASAP}_{\mathrm{sp}}$ (ours) & \textbf{94.69} & 69.22 & 66.00 & 54.65\\ %seed 45
$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & 94.50 & 68.76 & 66.60 & 56.12\\
\bottomrule              
\end{tabular}
\label{tab:adv_abl_rn9}
\end{center}
\end{table}

==> tab_compare_cc_abl.tex <==
\begin{table}[t]
\caption[]{Clean accuracy and accuracy common corruptions \cite{hendrycks2019robustness} (mean over all severties and corruptions) for ResNet-50 trained without adversarial training on ImageNet-1k. Comparision between \cite{vasconcelos2021impact} and our FLC and ASAP.
}
\begin{center}
\begin{tabular}{@{}l|cc@{}}
\toprule
 Method     &   Acc@1  &  Common Corruption\\ 
\toprule
% Baseline & 75.85  & 40.80  \\
% \midrule
\cite{vasconcelos2021impact} & 77.50  & 30.00 \\
\cite{vasconcelos2021impact} + RandAug \cite{cubuk2020randaugment} &  78.40 & 34.50 \\
\cite{vasconcelos2021impact} + Swish + RandAug \cite{cubuk2020randaugment} &  \textbf{78.80 }& 35.10 \\
\midrule
FLC Pooling (ours) &77.13  & 50.51    \\ 
$\mathrm{ASAP}_{\mathrm{stbl}}$ (ours) &77.12  & 50.76  \\ 
$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & 78.11 & 53.34 \\
$\mathrm{ASAP}_{\mathrm{sp}}$ (ours) & 78.54  & \textbf{54.20} \\
\bottomrule      
\end{tabular}
\label{tab:comp_cc_abl}
\end{center}
\end{table}

==> tab_pgd_only_imn1k.tex <==
\setlength{\tabcolsep}{1.2em}
%\noindent{\textbf{ImageNet.}} 
\begin{table}
\scriptsize
  \caption{%
  Comparison of ResNet-50 models that are trained non-adversarially or adversarially with PGD on ImageNet-1k.
  Accuracies (in percentage) shown on clean and perturbed (AutoAttack \cite{auto_attack}) validation images.
  We compare against models reported on RobustBench \cite{robust_bench}.}
    \centering
    \begin{tabular}{cl|cc}
    \toprule
    \multicolumn{2}{c|}{Method} & Clean & \makecell{AA $L_{\inf}$\\
    $\epsilon = \frac{4}{255}$} \\
    \midrule
    \multicolumn{2}{c|}{Non-adversarial training \cite{robust_bench}} & 76.52 & 0.00 \\
    \midrule
         \multirow{3}{*}{\rotatebox[origin=c]{90}{PGD}} & Robustness lib, 2019 \cite{robustness_github} & 62.56 & 29.22\\
         & Salman et al., 2020 \cite{salman2020adversarially} & 64.02 & 34.96\\
         & $\text{ASAP}_{\textrm{sp}}$ (ours)
         & 64.54 & 31.02 \\
         \bottomrule
    \end{tabular}
    \label{tab:imagenet_pgd_trained}
%\vspace{-20pt}
\end{table}

==> tab_robust_acc_cifar.tex <==
\begin{table}[t]
\caption[]{Accuracy for several state-of-the-art models trained without vadversarial training on CIFAR-10. We clearly can see, that our improved FLC pooling which neither suffers from aliasing nor from spectral artifacts, is natively more robust.
}
\begin{center}
\begin{tabular}{l|cccc}
\toprule
Name     &   Acc@1 &  APGD  &   FGSM &Squares\\
\toprule
ConvNeXt-tiny \cite{liu2022convnet} &   && \\
FLC  \cite{grabinski2022frequencylowcut} & & & \\
ASAF (ours) & &  & \\
\midrule
DenseNet-121 \cite{huang2017densely} & 94.24  &79.92& 83.71 &\textbf{83.28}\\
FLC  \cite{grabinski2022frequencylowcut} & 94.12&\textbf{79.94} & \textbf{83.93} & 81.21\\
ASAF (ours) &\textbf{94.44} & 78.55 & 83.18 &80.87\\
\midrule
ResNet-18    \cite{he2016deep}  &  93.21  & 73.33 & 79.11   & \textbf{79.85}     \\
FLC \cite{grabinski2022frequencylowcut} &  93.04  &75.94 & 78.91 &76.50 \\
ASAF (ours) &\textbf{93.58} &\textbf{76.11} &\textbf{79.25} & 77.61\\
\midrule
MobileNet-v2 \cite{sandler2018mobilenetv2}& 94.64  & 76.56 &  80.64&\textbf{77.99}\\
FLC \cite{grabinski2022frequencylowcut} & 94.47 &\textbf{78.76}& \textbf{81.10} &77.20\\
ASAF (ours) & \textbf{94.92} &  77.14&  80.70 & 76.77\\
\bottomrule              
\end{tabular}
\label{tab:imagenet_acc}
\end{center}
\end{table}

==> tab_stab_pad_abl_rebuttal.tex <==
\begin{table*}[t]
\caption[]{Accuracy (in percentage) and on clean samples, perturbed samples with FGSM~\cite{harnesssing} and PGD~\cite{pgd} as well as corrupted samples~\cite{hendrycks2019robustness} for different settings of ASAP on ResNet-18 \cite{he2016deep} trained without adversarial training on CIFAR-10. Attacks are done with an epsilon of $\epsilon=1/255$ and corruption performance is reported as mean over all severities.
}
\begin{center}
\begin{tabular}{l|@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c}
\toprule
Architecture  &   Acc@1 &  FGSM  &   PGD & Common Corruptions\\
\toprule
Baseline &  93.03 $\pm$ 0.13 & 78.62 $\pm$ 0.28 & 72.49 $\pm$ 0.67  & 76.93  $\pm$ 0.45    \\
$\mathrm{ASAP}_{\mathrm{stbl}}$(ours) & 93.12 $\pm$ 0.25 & 79.08 $\pm$ 0.43 & 75.06 $\pm$ 0.76 & \textbf{78.68 $\pm$ 0.19}\\
$\mathrm{ASAP}_{\mathrm{lp}}$ (ours) & \textbf{93.24 $\pm$ 0.15} & \textbf{79.17 $\pm$ 0.23} & 74.94 $\pm$ 0.56 & 78.65 $\pm$ 0.33\\
$\mathrm{ASAP}_{\mathrm{sp}}$(ours) &  93.00 $\pm$ 0.12 & 79.12 $\pm$ 0.49 & 74.69 $\pm$ 1.36 & 78.42 $\pm$ 0.20 \\
$\mathrm{ASAP}_{\mathrm{lp}}$ + stabilized FFT (ours) & 93.22 $\pm$ 0.07 & 78.37 $\pm$ 0.77  & \textbf{75.65 $\pm$ 1.43} &   78.38 $\pm$ 0.38 \\
$\mathrm{ASAP}_{\mathrm{sp}}$ + stabilized FFT (ours) & 92.88  $\pm$ 0.11 & 77.29 $\pm$ 1.02 & 74.82 $\pm$    1.90 & 78.77 $\pm$ 0.17 \\
\bottomrule              
\end{tabular}
\label{tab:stab_pad_abl}
\end{center}
\end{table*}
